Space-Time-Separable Graph Convolutional Network for Pose Forecasting

Human pose forecasting is a complex structured-data sequence-modelling task, which has received increasing attention, also due to numerous potential applications. Research has mainly addressed the temporal dimension as time series and the interaction of human body joints with a kinematic tree or by a graph. This has decoupled the two aspects and leveraged progress from the relevant fields, but it has also limited the understanding of the complex structural joint spatio-temporal dynamics of the human pose. Here we propose a novel Space-Time-Separable Graph Convolutional Network (STS-GCN) for pose forecasting. For the first time, STS-GCN models the human pose dynamics only with a graph convolutional network (GCN), including the temporal evolution and the spatial joint interaction within a single-graph framework, which allows the cross-talk of motion and spatial correlations. Concurrently, STS-GCN is the first space-time-separable GCN: the space-time graph connectivity is factored into space and time affinity matrices, which bottlenecks the space-time cross-talk, while enabling full joint-joint and time-time correlations. Both affinity matrices are learnt end-to-end, which results in connections substantially deviating from the standard kinematic tree and the linear-time time series. In experimental evaluation on three complex, recent and large-scale benchmarks, Human3.6M [Ionescu et al. TPAMI'14], AMASS [Mahmood et al. ICCV'19] and 3DPW [Von Marcard et al. ECCV'18], STS-GCN outperforms the state-of-the-art, surpassing the current best technique [Mao et al. ECCV'20] by over 32% in average at the most difficult long-term predictions, while only requiring 1.7% of its parameters. We explain the results qualitatively and illustrate the graph interactions by the factored joint-joint and time-time learnt graph connections. Our source code is available at: https://github.com/FraLuca/STSGCN

==> Sections/4.Results.tex <==
\section{Results}
To be consistent with the literature, we report our results for short-term ($<500ms$) and long-term ($>500ms$) predictions. We will also provide visualizations of our models’ predictions for both of our datasets, for assessing intuitively their quality.\\



\input{Sections/Table/long_mm}




\begin{figure*}[h!]
\begin{center}
\includegraphics[width=0.95\textwidth]{images/25_walking_line.png}
\end{center}
   \caption{25 frames walking}
\label{fig:short}
\end{figure*}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{images/25_walking_grid.png}
\end{center}
   \caption{25 frames walking}
\label{fig:short}
\end{figure}




\begin{figure*}[ht]
  \begin{minipage}[t]{500pt}
    \includegraphics[width=.98\textwidth, height=0.07\textwidth]{images/walk_25.png}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{500pt}
    \includegraphics[width=.98\textwidth, height=0.06\textwidth]{images/discuss_25.png}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{500pt}
    \includegraphics[width=.98\textwidth, height=0.07\textwidth]{images/posing_25.png}
  \end{minipage}
  \caption{25 frames prediction on Human3.6M action \textit{walking} (top), \textit{discussion} (middle) and \textit{posing} (bottom). The purple-green
skeleton (for right and left parts of the body respectively) is our prediction while the
gray-black dotted-lines-skeleton is the ground truth of our predictions. The action \textit{posing} (line3) shows our failure case, the pose is accurate in the initial frames but the prediction loses motion amplitude as the output frames get longer (10.3 cm loss). Line1 shows the periodic \textit{walking} action,  the prediction has a precise match with the ground truth for each predicted frame, the loss is 5 centimeters. For the aperiodic action \textit{discussion} (line2) has an error of 7.8 centimetres.  The upper limbs lose prediction accuracy over time, but our pose fits the ground truth for each frame.}
\label{fig:seq_pred}
\end{figure*}


\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.35\textwidth]{images/space_conn.PNG}
\end{center}
   \caption{A sample of spatial connections learnt.Some predictions are positive or large positive (in green) while some are negative or large negative (in orange). Weak connections have not been taken into account. Connections are present along the kinematic tree even if in this sample the central part of the body is poorly connected. Some connections between non-adjacent joints are interesting, such as the left foot with the neck, or the head with the left hand. We note how both hands are characterised by a large positive connection with themselves. \fab{not clear. I guess you may want to use the term ``along the kinematic tree'', or ``coincide with the kinematic tree'' (but not always, it seems. In other words you may want to say that the tree is effectively important, but there are other important connections too. Also: need to comment on positive and negative values and the anti-correlation, if one may say so.}
   }
   \theo {i think in order to understand the negative correlations,we must understand the coordinates that we are predicting for each body joint. The coordinates are relative to the pelvis, which is always in the position [0,0,0], for all the frames. Thus, the coordinates of the other body parts are relative to the pelvis, not 'general' coordinates from a standard vantage point. My intuition, and i could be wrong, is that we care for the strong connections, in absolute values. The + or - signs depends on whether the coordinates of 2 body joints,that form a connection, are both positive,negative or one is positive and the other is negative}
\label{fig:spat_conn}
\end{figure}



\captionsetup[subfloat]{labelformat=empty}
  \subfloat[Learnt $A^s$ (layer 1, time 1)]{\includegraphics[width=.215\textwidth]{images/time_space.pdf} }
\subfloat[Learnt $A^t$ (layer 1, head)]{\includegraphics[width=.22\textwidth]{images/time_space2.pdf} }



\captionsetup[subfloat]{labelformat=empty}
\subfloat[Walking\label{fig:seq1}]{\includegraphics[width=.85\textwidth, height=0.10\textwidth]{images/walking.pdf} }
\newline
\subfloat[Discussion\label{fig:seq2}]{\includegraphics[width=.49\textwidth, height=0.1\textwidth]{images/discussion13.pdf} }
\hfill
\subfloat[Posing\label{fig:seq3}]{\includegraphics[width=.49\textwidth, height=0.1\textwidth]{images/posing13.pdf} }

==> Sections/Table/ablation2.tex <==


% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h!]
\centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{ccc|cccccccc|}
\cline{4-11}
 &
   &
  \multicolumn{1}{c}{} &
  \multicolumn{8}{|c|}{Average} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular} [c] {@{}c@{}}One\\ Convolution\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular} [c]{@{}c@{}} Shared\\ Matrices\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Factorised \\ Graph\end{tabular}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{240}} &
  {\ul \textit{400}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} \\ \midrule
\multicolumn{1}{|c}{} &
   &
  $\bullet$ &
  30.3 &
  27.2 &
  40.0 &
  48.3 &
  57.9 &
  66.0 &
  73.9 &
  79.7 \\
\multicolumn{1}{|c}{$\bullet$} &
  $\bullet$ &
  $\bullet$ &
  11.3 &
  18.7 &
  31.9 &
  38.9 &
  51.9 &
  61.3 &
  \textbf{69.7} &
  75.3 \\ 
\multicolumn{1}{|c}{$\bullet$} &
   &
   &
  13.0 &
  22.3 &
  33.5 &
  40.3 &
  52.9 &
  63.4 &
  76.3 &
  77.1 \\ 
\multicolumn{1}{|c}{$\bullet$} &
   &
  $\bullet$ &
  \textbf{9.8} &
  \textbf{17.3} &
  \textbf{31.2} &
  \textbf{36.3} &
  \textbf{49.1} &
  \textbf{59.6} &
  \textbf{69.7} &
  \textbf{74.7} \\ \bottomrule
\end{tabular}}
\caption{Ablation study on Human3.6, mm}
\label{tab:ablation2}
\end{table}

==> Sections/Table/angle_avg_8sub.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h!]
\centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{|c|cccccccc|}
\cline{2-9}

\multicolumn{1}{l|}{} &
  \multicolumn{8}{c|}{Average} \\ \hline

\multicolumn{1}{|c|}{\textit{ms}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} \\ \cline{1-9}
LTD-10-25 \cite{Mao19LTD} &
  0.30 &
  0.54 &
  0.86 &
  0.97 &
  1.15 &
  1.29 &
  1.48 &
  1.59 \\

LTD-10-10 \cite{Mao19LTD} &
  0.27 &
  0.52 &
  0.83 &
  0.95 &
  1.16 &
  1.32 &
  1.51 &
  1.62 \\

BC-WGAIL-div \cite{Wang19} &
  0.31 &
  0.57 &
  0.90 &
  1.02 &
  1.23 &
  - &
  - &
  1.65 \\

DCT-RNN-GCN \cite{Mao20DCT} &
  0.27 &
  0.52 &
  0.82 &
  0.94 &
  1.14 &
  1.28 &
  1.46 &
  1.57 \\ \cline{1-9}

\multicolumn{1}{|c|}{Ours} &
  \textbf{0.23} &
  \textbf{0.37} &
  \textbf{0.58} &
  \textbf{0.65} &
  \textbf{0.80} &
  \textbf{0.90} &
  \textbf{1.02} &
  \textbf{1.12} \\ \bottomrule
\end{tabular}}
\caption{Prediction of joint angles on Human3.6M}
\label{tab:angle_avg8}
\end{table}

==> Sections/Table/long_ang_256sub.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[!htb]
\centering
\resizebox{.7\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|}
\cline{2-17}
\multicolumn{1}{l|}{\textbf{}} &
  \multicolumn{4}{c|}{Walking} &
  \multicolumn{4}{c|}{Eating} &
  \multicolumn{4}{c|}{Smoking} &
  \multicolumn{4}{c|}{Discussion} \\ \hline
\multicolumn{1}{|c|}{\textit{msec}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} \\ \cline{1-17}
LTD-10-25  \cite{Mao19LTD}  & 0.92 & 0.97 & 1.03 & 1.05 & 0.99 & 1.16 & 1.26 & 1.33 & 1.07 & 1.26 & 1.41 & 1.55 & 1.48 & 1.59 & 1.68 & 1.76 \\
LTD-10-10 \cite{Mao19LTD}   & 0.95 & 1.03 & 1.09 & 1.12 & 0.98 & 1.15 & 1.28 & 1.36 & 1.04 & 1.21 & 1.36 & 1.51 & 1.47 & 1.59 & 1.71 & 1.79 \\
BC-WGAIL-div \cite{Wang19} & 0.67 & -    & -    & \textbf{0.69} & 0.79 & -    & -    & 1.13 & 0.95 & -    & -    & 1.63 & 1.34 & -    & -    & 1.81 \\
DCT-RNN-GCN \cite{Mao20DCT}   & 0.84 & 0.91 & 0.99 & 1.03 & 0.98 & 1.14 & 1.24 & 1.31 & 1.04 & 1.20 & 1.38 & 1.50 & 1.49 & 1.62 & 1.72 & 1.82 \\ \cline{1-17}
\multicolumn{1}{|c|}{Ours} &
  \textbf{0.47} &
  \textbf{0.56} &
  \textbf{0.60} &
  0.61 &
  \textbf{0.50} &
  \textbf{0.60} &
  \textbf{0.65} &
  \textbf{0.72} &
  \textbf{0.65} &
  \textbf{0.73} &
  \textbf{0.83} &
  \textbf{0.89} &
  \textbf{0.87} &
  \textbf{0.97} &
  \textbf{1.14} &
  \textbf{1.15} \\ \bottomrule
\end{tabular}}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|cccc|cccc|}
\cline{2-25}
\multicolumn{1}{l|}{} &
  \multicolumn{4}{c|}{Directions} &
  \multicolumn{4}{c|}{Greeting} &
  \multicolumn{4}{c|}{Phoning} &
  \multicolumn{4}{c|}{Posing} &
  \multicolumn{4}{c|}{Purchases} &
  \multicolumn{4}{c|}{Sitting} \\ \hline
\multicolumn{1}{|c|}{\textit{msec}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} \\ \cline{1-25}
LTD-10-25 \cite{Mao19LTD} &
  1.10 &
  1.23 &
  1.35 &
  1.41 &
  1.63 &
  1.81 &
  1.95 &
  2.01 &
  1.29 &
  1.48 &
  1.63 &
  1.74 &
  1.54 &
  1.81 &
  2.10 &
  2.23 &
  1.51 &
  1.66 &
  1.80 &
  1.87 &
  1.34 &
  1.60 &
  1.79 &
  1.87 \\
LTD-10-10 \cite{Mao19LTD} &
  1.09 &
  1.21 &
  1.34 &
  1.41 &
  1.63 &
  1.82 &
  1.99 &
  2.06 &
  1.29 &
  1.50 &
  1.67 &
  1.78 &
  1.53 &
  1.81 &
  2.12 &
  2.25 &
  1.52 &
  1.68 &
  1.83 &
  1.91 &
  1.34 &
  1.60 &
  1.79 &
  1.89 \\
BC-WGAIL-div \cite{Wang19} &
  0.95 &
  - &
  - &
  1.41 &
  1.62 &
  - &
  - &
  1.72 &
  1.56 &
  - &
  - &
  1.67 &
  1.83 &
  - &
  - &
  2.69 &
  1.46 &
  - &
  - &
  2.23 &
  1.21 &
  - &
  - &
  1.58 \\
DCT-RNN-GCN \cite{Mao20DCT} &
  1.08 &
  1.22 &
  1.35 &
  1.42 &
  1.62 &
  1.79 &
  1.93 &
  1.99 &
  1.28 &
  1.49 &
  1.65 &
  1.76 &
  1.55 &
  1.80 &
  2.10 &
  2.24 &
  1.47 &
  1.62 &
  1.75 &
  1.82 &
  1.33 &
  1.59 &
  1.79 &
  1.88 \\ \cline{1-25}
\multicolumn{1}{|c|}{Ours} &
  \textbf{0.60} &
  \textbf{0.71} &
  \textbf{0.81} &
  \textbf{0.83} &
  \textbf{0.99} &
  \textbf{1.09} &
  \textbf{1.22} &
  \textbf{1.32} &
  \textbf{1.15} &
  \textbf{1.22} &
  \textbf{1.24} &
  \textbf{1.26} &
  \textbf{0.97} &
  \textbf{1.28} &
  \textbf{1.39} &
  \textbf{1.71} &
  \textbf{0.95} &
  \textbf{1.11} &
  \textbf{1.24} &
  \textbf{1.33} &
  \textbf{0.78} &
  \textbf{0.89} &
  \textbf{0.95} &
  \textbf{1.05} \\ \bottomrule
\end{tabular}}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|cccc|cccc|}
\cline{2-25}
\multicolumn{1}{l|}{} &
  \multicolumn{4}{c|}{Sitting Down} &
  \multicolumn{4}{c|}{Taking Photo} &
  \multicolumn{4}{c|}{Waiting} &
  \multicolumn{4}{c|}{Walking Dog} &
  \multicolumn{4}{c|}{Walking Together} &
  \multicolumn{4}{c|}{Average} \\ \hline
\multicolumn{1}{|c|}{\textit{msec}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} \\ \cline{1-25}
LTD-10-25 \cite{Mao19LTD}&
  1.71 &
  1.95 &
  2.17 &
  2.26 &
  0.94 &
  1.10 &
  1.23 &
  1.34 &
  1.30 &
  1.48 &
  1.63 &
  1.74 &
  1.30 &
  1.45 &
  1.55 &
  1.64 &
  0.91 &
  0.98 &
  1.02 &
  1.06 &
  1.27 &
  1.44 &
  1.57 &
  1.66 \\
LTD-10-10 \cite{Mao19LTD} &
  1.68 &
  1.91 &
  2.13 &
  2.22 &
  0.93 &
  1.08 &
  1.22 &
  1.34 &
  1.30 &
  1.47 &
  1.63 &
  1.75 &
  1.31 &
  1.48 &
  1.59 &
  1.68 &
  0.89 &
  0.98 &
  1.03 &
  1.08 &
  1.26 &
  1.44 &
  1.59 &
  1.68 \\
BC-WGAIL-div \cite{Wang19} &
  1.34 &
  - &
  - &
  1.78 &
  0.84 &
  - &
  - &
  1.06 &
  1.59 &
  - &
  - &
  2.39 &
  1.65 &
  - &
  - &
  1.86 &
  0.67 &
  - &
  - &
  1.15 &
  1.23 &
  - &
  - &
  1.65 \\
DCT-RNN-GCN \cite{Mao20DCT} &
  1.68 &
  1.90 &
  2.12 &
  2.22 &
  0.92 &
  1.07 &
  1.21 &
  1.33 &
  1.31 &
  1.49 &
  1.64 &
  1.77 &
  1.30 &
  1.45 &
  1.55 &
  1.63 &
  0.86 &
  0.94 &
  1.00 &
  1.04 &
  1.25 &
  1.42 &
  1.56 &
  1.65 \\ \cline{1-25}
\multicolumn{1}{|c|}{Ours} &
  \textbf{0.86} &
  \textbf{1.04} &
  \textbf{1.09} &
  \textbf{1.22} &
  \textbf{0.62} &
  \textbf{0.69} &
  \textbf{0.76} &
  \textbf{0.79} &
  \textbf{0.88} &
  \textbf{1.08} &
  \textbf{1.22} &
  \textbf{1.32} &
  \textbf{1.09} &
  \textbf{1.24} &
  \textbf{1.32} &
  \textbf{1.39} &
  \textbf{0.51} &
  \textbf{0.58} &
  \textbf{0.60} &
  \textbf{0.69} &
  \textbf{0.79} &
  \textbf{0.92} &
  \textbf{1.00} &
  \textbf{1.09} \\ \bottomrule
\end{tabular}}
\caption{
MAE error in degree for the long-term prediction of Euler's angles of the joint positions on Human3.6M.
Refer to Sec.~\ref{secsm:angles} for a discussion.
%Average improvement on the different actions is at least 27\%
}
\label{tab:ang_long}
\end{table*}



==> Sections/Table/long_ang_8sub.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|}
\cline{2-17}
\multicolumn{1}{l|}{\textbf{}} &
  \multicolumn{4}{c|}{Walking} &
  \multicolumn{4}{c|}{Eating} &
  \multicolumn{4}{c|}{Smoking} &
  \multicolumn{4}{c|}{Discussion} \\ \hline
\multicolumn{1}{|c|}{\textit{ms}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} \\ \cline{1-17}
LTD-10-25 \cite{Mao19LTD}   & 0.65 & 0.69 & 0.69 & 0.67 & 0.76 & 0.82 & 1.00 & 1.12 & 0.87 & 0.99 & 1.33 & 1.57 & 1.33 & 1.53 & 1.62 & 1.70 \\
LTD-10-10 \cite{Mao19LTD}   & 0.69 & 0.77 & 0.76 & 0.77 & 0.76 & 0.81 & 1.00 & 1.10 & 0.88 & 1.01 & 1.36 & 1.58 & 1.27 & 1.51 & 1.66 & 1.75 \\
BC-WGAIL-div \cite{Wang19} & 0.67 & -    & -    & 0.69 & 0.79 & -    & -    & 1.13 & 0.95 & -    & -    & 1.63 & 1.34 & -    & -    & 1.81 \\
DCT-RNN-GCN \cite{Mao20DCT}    & 0.59 & 0.62 & 0.61 & 0.64 & 0.74 & 0.81 & 1.01 & 1.10 & 0.86 & 1.00 & 1.35 & 1.58 & 1.29 & 1.51 & 1.61 & 1.63 \\ \cline{1-17}
\multicolumn{1}{|c|}{Ours} &
  \textbf{0.47} &
  \textbf{0.54} &
  \textbf{0.60} &
  \textbf{0.61} &
  \textbf{0.51} &
  \textbf{0.58} &
  \textbf{0.66} &
  \textbf{0.78} &
  \textbf{0.64} &
  \textbf{0.73} &
  \textbf{0.83} &
  \textbf{0.97} &
  \textbf{0.92} &
  \textbf{0.96} &
  \textbf{1.13} &
  \textbf{1.17} \\ \bottomrule
\end{tabular}}
\end{table*}



\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|cccc|cccc|}
\cline{2-25}
\multicolumn{1}{l|}{} &
  \multicolumn{4}{c|}{Directions} &
  \multicolumn{4}{c|}{Greeting} &
  \multicolumn{4}{c|}{Phoning} &
  \multicolumn{4}{c|}{Posing} &
  \multicolumn{4}{c|}{Purchases} &
  \multicolumn{4}{c|}{Sitting} \\ \hline
\multicolumn{1}{|c|}{\textit{ms}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} \\ \cline{1-25}
LTD-10-25 \cite{Mao19LTD} &
  0.84 &
  1.02 &
  1.23 &
  1.26 &
  1.43 &
  1.44 &
  1.59 &
  1.59 &
  1.45 &
  1.57 &
  1.66 &
  1.65 &
  1.62 &
  1.94 &
  2.22 &
  2.42 &
  1.42 &
  1.48 &
  1.93 &
  2.21 &
  1.08 &
  1.20 &
  1.39 &
  1.45 \\
LTD-10-10 \cite{Mao19LTD}&
  0.90 &
  1.07 &
  1.32 &
  1.35 &
  1.47 &
  1.47 &
  1.63 &
  1.59 &
  1.49 &
  1.64 &
  1.75 &
  1.74 &
  1.61 &
  2.02 &
  2.35 &
  2.55 &
  1.47 &
  1.57 &
  1.99 &
  2.27 &
  1.12 &
  1.25 &
  1.46 &
  1.52 \\
BC-WGAIL-div \cite{Wang19}&
  0.95 &
  - &
  - &
  1.41 &
  1.62 &
  - &
  - &
  1.72 &
  1.56 &
  - &
  - &
  1.67 &
  1.83 &
  - &
  - &
  2.69 &
  1.46 &
  - &
  - &
  2.23 &
  1.21 &
  - &
  - &
  1.58 \\
DCT-RNN-GCN \cite{Mao20DCT} &
  0.81 &
  1.02 &
  1.22 &
  1.27 &
  1.47 &
  1.47 &
  1.61 &
  1.57 &
  1.41 &
  1.55 &
  1.68 &
  1.68 &
  1.60 &
  1.78 &
  2.10 &
  2.32 &
  1.43 &
  1.53 &
  1.94 &
  2.22 &
  1.16 &
  1.29 &
  1.50 &
  1.55 \\ \cline{1-25}
\multicolumn{1}{|c|}{Ours} &
  \textbf{0.61} &
  \textbf{0.67} &
  \textbf{0.77} &
  \textbf{0.88} &
  \textbf{0.99} &
  \textbf{1.10} &
  \textbf{1.23} &
  \textbf{1.32} &
  \textbf{1.15} &
  \textbf{1.20} &
  \textbf{1.27} &
  \textbf{1.31} &
  \textbf{1.06} &
  \textbf{1.32} &
  \textbf{1.52} &
  \textbf{1.67} &
  \textbf{0.96} &
  \textbf{1.09} &
  \textbf{1.20} &
  \textbf{1.35} &
  \textbf{0.78} &
  \textbf{0.85} &
  \textbf{0.99} &
  \textbf{1.08} \\ \bottomrule
\end{tabular}}
\end{table*}


\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|cccc|cccc|}
\cline{2-25}
\multicolumn{1}{l|}{} &
  \multicolumn{4}{c|}{Sitting Down} &
  \multicolumn{4}{c|}{Taking Photo} &
  \multicolumn{4}{c|}{Waiting} &
  \multicolumn{4}{c|}{Walking Dog} &
  \multicolumn{4}{c|}{Walking Together} &
  \multicolumn{4}{c|}{Average} \\ \hline
\multicolumn{1}{|c|}{\textit{ms}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} &
  {\ul \textit{560}} &
  {\ul \textit{720}} &
  {\ul \textit{880}} &
  {\ul \textit{1000}} \\ \cline{1-25}
LTD-10-25 \cite{Mao19LTD} &
  1.26 &
  1.54 &
  1.70 &
  1.87 &
  0.85 &
  0.92 &
  0.99 &
  1.06 &
  1.55 &
  1.89 &
  2.20 &
  2.29 &
  1.52 &
  1.63 &
  1.78 &
  1.84 &
  0.70 &
  0.75 &
  0.82 &
  1.16 &
  1.15 &
  1.29 &
  1.48 &
  1.59 \\
LTD-10-10 \cite{Mao19LTD}&
  1.17 &
  1.40 &
  1.54 &
  1.67 &
  0.81 &
  0.89 &
  0.97 &
  1.05 &
  1.57 &
  1.94 &
  2.29 &
  2.37 &
  1.58 &
  1.66 &
  1.80 &
  1.86 &
  0.65 &
  0.73 &
  0.81 &
  1.16 &
  1.16 &
  1.32 &
  1.51 &
  1.62 \\
BC-WGAIL-div \cite{Li18} &
  1.34 &
  - &
  - &
  1.78 &
  0.84 &
  - &
  - &
  1.06 &
  1.59 &
  - &
  - &
  2.39 &
  1.65 &
  - &
  - &
  1.86 &
  0.67 &
  - &
  - &
  1.15 &
  1.23 &
  - &
  - &
  1.65 \\
DCT-RNN-GCN \cite{Mao20DCT} &
  1.18 &
  1.42 &
  1.55 &
  1.70 &
  0.82 &
  0.91 &
  1.00 &
  1.08 &
  1.54 &
  1.90 &
  2.22 &
  2.30 &
  1.57 &
  1.63 &
  1.76 &
  1.82 &
  0.63 &
  0.68 &
  0.79 &
  1.16 &
  1.14 &
  1.28 &
  1.46 &
  1.57 \\ \cline{1-25}
\multicolumn{1}{|c|}{Ours} &
  \textbf{0.88} &
  \textbf{1.03} &
  \textbf{1.24} &
  \textbf{1.33} &
  \textbf{0.59} &
  \textbf{0.65} &
  \textbf{0.72} &
  \textbf{0.83} &
  \textbf{0.84} &
  \textbf{1.02} &
  \textbf{1.17} &
  \textbf{1.30} &
  \textbf{1.12} &
  \textbf{1.23} &
  \textbf{1.30} &
  \textbf{1.46} &
  \textbf{0.49} &
  \textbf{0.57} &
  \textbf{0.65} &
  \textbf{0.67} &
  \textbf{0.80} &
  \textbf{0.90} &
  \textbf{1.02} &
  \textbf{1.12} \\ \bottomrule
\end{tabular}}
\caption{Long Term, Euler on Human3.6}
\label{tab:long_ang}
\end{table*}




==> Sections/Table/short_ang_256sub.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}



\begin{table*}[!htb]
\centering
\resizebox{.7\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|}
\cline{2-17}
\multicolumn{1}{l|}{} &
  \multicolumn{4}{c|}{Walking} &
  \multicolumn{4}{c|}{Eating} &
  \multicolumn{4}{c|}{Smoking} &
  \multicolumn{4}{c|}{Discussion} \\ \hline
\multicolumn{1}{|c|}{\textit{msec}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} \\ \cline{1-17}
LTD-10-25 \cite{Mao19LTD}   & 0.26          & 0.47 & 0.73 & 0.80 & 0.21          & 0.45 & 0.71 & 0.82 & 0.26 & 0.43 & 0.74 & 0.86 & 0.48          & 0.67 & 1.10 & 1.28 \\
LTD-10-10 \cite{Mao19LTD}   & 0.25          & 0.45 & 0.72 & 0.78 & 0.20          & 0.41 & 0.70 & 0.82 & 0.25 & 0.41 & 0.71 & 0.83 & 0.47          & 0.68 & 1.09 & 1.25 \\
BC+WGAIL-div \cite{Wang19} & 0.21 & 0.34 & 0.53 & 0.59 & 0.17 & 0.30 & 0.52 & 0.65 & 0.23 & 0.44 & 0.87 & 0.85 & 0.23 & 0.56 & 0.82 & 0.91 \\
DCT-RNN-GCN \cite{Mao20DCT}    & 0.24          & 0.43 & 0.66 & 0.71 & 0.20          & 0.41 & 0.68 & 0.80 & 0.25 & 0.41 & 0.71 & 0.83 & 0.44          & 0.68 & 1.09 & 1.25 \\ \cline{1-17}
\multicolumn{1}{|c|}{Ours} &
  \textbf{0.18} &
  \textbf{0.24} &
  \textbf{0.36} &
  \textbf{0.40} &
  \textbf{0.15} &
  \textbf{0.22} &
  \textbf{0.34} &
  \textbf{0.41} &
  \textbf{0.18} &
  \textbf{0.28} &
  \textbf{0.48} &
  \textbf{0.55} &
  0.20 &
  \textbf{0.40} &
  \textbf{0.67} &
  \textbf{0.74} \\ \bottomrule
\end{tabular}}
\end{table*}



% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|cccc|cccc|}
\cline{2-25}
\multicolumn{1}{l|}{} &
  \multicolumn{4}{c|}{Directions} &
  \multicolumn{4}{c|}{Greeting} &
  \multicolumn{4}{c|}{Phoning} &
  \multicolumn{4}{c|}{Posing} &
  \multicolumn{4}{c|}{Purchases} &
  \multicolumn{4}{c|}{Sitting} \\ \hline
\multicolumn{1}{|c|}{\textit{msec}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} \\ \cline{1-25}
LTD-10-25 \cite{Mao19LTD} &
  0.20 &
  0.41 &
  0.76 &
  0.92 &
  0.52 &
  0.84 &
  1.24 &
  1.41 &
  0.34 &
  0.57 &
  0.96 &
  1.09 &
  0.31 &
  0.60 &
  1.06 &
  1.24 &
  0.47 &
  0.84 &
  1.24 &
  1.33 &
  0.33 &
  0.52 &
  0.92 &
  1.06 \\
LTD-10-10 \cite{Mao19LTD} &
  \textbf{0.19} &
  0.39 &
  0.75 &
  0.91 &
  0.53 &
  0.82 &
  1.22 &
  1.39 &
  0.33 &
  \textbf{0.54} &
  \textbf{0.94} &
  \textbf{1.07} &
  0.30 &
  0.61 &
  1.02 &
  1.20 &
  0.45 &
  0.80 &
  1.22 &
  1.32 &
  0.28 &
  0.56 &
  0.94 &
  1.08 \\
BC+WGAIL-div \cite{Wang19}&
  0.27 &
  0.46 &
  0.81 &
  0.89 &
  0.43 &
  0.75 &
  1.17 &
  1.33 &
  0.54 &
  1.05 &
  1.40 &
  1.56 &
  0.27 &
  0.55 &
  1.16 &
  1.41 &
  0.54 &
  0.78 &
  1.07 &
  1.14 &
  0.29 &
  0.48 &
  0.87 &
  1.04 \\
DCT-RNN-GCN \cite{Mao20DCT} &
  \textbf{0.19} &
  0.38 &
  0.74 &
  0.90 &
  0.50 &
  0.79 &
  1.21 &
  1.38 &
  \textbf{0.32} &
  \textbf{0.54} &
  \textbf{0.94} &
  \textbf{1.07} &
  0.27 &
  0.57 &
  1.00 &
  1.22 &
  0.43 &
  0.80 &
  1.22 &
  1.32 &
  0.28 &
  0.56 &
  0.94 &
  1.06 \\ \cline{1-25}
\multicolumn{1}{|c|}{Ours} &
  0.22 &
  \textbf{0.33} &
  \textbf{0.49} &
  \textbf{0.51} &
  \textbf{0.28} &
  \textbf{0.46} &
  \textbf{0.71} &
  \textbf{0.78} &
  0.35 &
  0.70 &
  0.97 &
  \textbf{1.07} &
  \textbf{0.21} &
  \textbf{0.42} &
  \textbf{0.67} &
  \textbf{0.87} &
  \textbf{0.39} &
  \textbf{0.57} &
  \textbf{0.77} &
  \textbf{0.81} &
  \textbf{0.23} &
  \textbf{0.36} &
  \textbf{0.54} &
  \textbf{0.61} \\ \bottomrule
\end{tabular}}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|cccc|cccc|}
\cline{2-25}
\multicolumn{1}{l|}{} &
   \multicolumn{4}{c|}{Sitting Down} &
  \multicolumn{4}{c|}{Taking Photo} &
  \multicolumn{4}{c|}{Waiting} &
  \multicolumn{4}{c|}{Walking Dog} &
  \multicolumn{4}{c|}{Walking Together} &
  \multicolumn{4}{c|}{Average} \\ \hline
\multicolumn{1}{|c|}{\textit{msec}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} \\ \cline{1-25}
LTD-10-25 \cite{Mao19LTD} &
  0.44 &
  0.75 &
  1.21 &
  1.40 &
  0.21 &
  0.35 &
  0.62 &
  0.74 &
  0.29 &
  0.49 &
  0.92 &
  1.07 &
  0.44 &
  0.71 &
  1.04 &
  1.14 &
  0.26 &
  0.43 &
  0.67 &
  0.77 &
  0.34 &
  0.57 &
  0.93 &
  1.06 \\
LTD-10-10 \cite{Mao19LTD} &
  0.43 &
  0.74 &
  1.20 &
  1.38 &
  0.20 &
  0.34 &
  0.61 &
  0.72 &
  0.28 &
  0.47 &
  0.90 &
  1.05 &
  0.43 &
  0.69 &
  1.02 &
  1.13 &
  0.24 &
  0.40 &
  0.63 &
  0.73 &
  0.32 &
  0.55 &
  0.91 &
  1.04 \\
BC+WGAIL-div \cite{Wang19}&
  \textbf{0.34} &
  0.68 &
  1.01 &
  1.14 &
  0.17 &
  0.37 &
  0.60 &
  0.72 &
  0.25 &
  0.53 &
  0.96 &
  1.19 &
  0.46 &
  0.80 &
  1.12 &
  1.31 &
  0.19 &
  0.41 &
  0.61 &
  0.64 &
  0.31 &
  0.57 &
  0.90 &
  1.02 \\
DCT-RNN-GCN \cite{Mao20DCT} &
  0.43 &
  0.74 &
  1.20 &
  1.39 &
  0.19 &
  0.34 &
  0.60 &
  0.72 &
  0.27 &
  0.47 &
  0.91 &
  1.07 &
  0.42 &
  0.68 &
  1.01 &
  1.12 &
  0.24 &
  0.39 &
  0.62 &
  0.71 &
  0.31 &
  0.55 &
  0.90 &
  1.04 \\ \cline{1-25}
\multicolumn{1}{|c|}{Ours} &
  0.23 &
  \textbf{0.44} &
  \textbf{0.66} &
  \textbf{0.73} &
  \textbf{0.15} &
  \textbf{0.26} &
  \textbf{0.41} &
  \textbf{0.47} &
  \textbf{0.20} &
  \textbf{0.34} &
  \textbf{0.56} &
  \textbf{0.66} &
  \textbf{0.40} &
  \textbf{0.63} &
  \textbf{0.85} &
  \textbf{0.92} &
  \textbf{0.16} &
  \textbf{0.26} &
  \textbf{0.37} &
  \textbf{0.42} &
  \textbf{0.24} &
  \textbf{0.39} &
  \textbf{0.59} &
  \textbf{0.66} \\ \bottomrule
\end{tabular}}
\caption{MAE error in degree for the short-term prediction of Euler's angles of the joint positions on Human3.6M.Refer to Sec.~\ref{secsm:angles} for a discussion.}
%Average improvement on the different actions is at least 19\%
%\ale{19.4 for 2frames, at least 29.1 from 4frames}
\label{tab:ang_short}
\end{table*}


==> Sections/Table/short_ang_8sub.tex <==
% SHORT EULER

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|}
\cline{2-17}
\multicolumn{1}{l|}{} &
  \multicolumn{4}{c|}{Walking} &
  \multicolumn{4}{c|}{Eating} &
  \multicolumn{4}{c|}{Smoking} &
  \multicolumn{4}{c|}{Discussion} \\ \hline
\multicolumn{1}{|c|}{\textit{ms}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} \\ \cline{1-17}
  
LTD-10-10 \cite{Mao19LTD}   & 0.18 & 0.31 & 0.49 & 0.56 & 0.16 & 0.29 & 0.50 & 0.62 & 0.22 & 0.41 & 0.86 & 0.80 & \textbf{0.20} & 0.51 & 0.77 & 0.85 \\
BC+WGAIL-div \cite{Wang19} & 0.21 & 0.34 & 0.53 & 0.59 & 0.17 & 0.30 & 0.52 & 0.65 & 0.23 & 0.44 & 0.87 & 0.85 & 0.23          & 0.56 & 0.82 & 0.91 \\
DCT-RNN-GCN \cite{Mao20DCT}    & 0.18 & 0.30 & 0.46 & 0.51 & 0.16 & 0.29 & 0.49 & 0.60 & 0.22 & 0.42 & 0.86 & 0.80 & \textbf{0.20} & 0.52 & 0.78 & 0.87 \\ \cline{1-17}
\multicolumn{1}{|c|}{Ours} &
  \textbf{0.16} &
  \textbf{0.23} &
  \textbf{0.34} &
  \textbf{0.40} &
  \textbf{0.15} &
  \textbf{0.21} &
  \textbf{0.35} &
  \textbf{0.40} &
  \textbf{0.18} &
  \textbf{0.27} &
  \textbf{0.48} &
  \textbf{0.56} &
  \textbf{0.20} &
  \textbf{0.39} &
  \textbf{0.71} &
  \textbf{0.71} \\ \bottomrule
\end{tabular}}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|cccc|cccc|}
\cline{2-25}
\multicolumn{1}{l|}{} &
  \multicolumn{4}{c|}{Directions} &
  \multicolumn{4}{c|}{Greeting} &
  \multicolumn{4}{c|}{Phoning} &
  \multicolumn{4}{c|}{Posing} &
  \multicolumn{4}{c|}{Purchases} &
  \multicolumn{4}{c|}{Sitting} \\ \hline
\multicolumn{1}{|c|}{\textit{ms}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} \\ \cline{1-25}
LTD-10-10 \cite{Mao19LTD} &
  0.26 &
  0.45 &
  0.71 &
  0.79 &
  0.36 &
  0.60 &
  0.95 &
  1.13 &
  0.53 &
  1.02 &
  1.35 &
  1.48 &
  0.19 &
  0.44 &
  1.01 &
  1.24 &
  0.43 &
  0.65 &
  1.05 &
  1.13 &
  0.29 &
  0.45 &
  0.80 &
  0.97 \\
BC+WGAIL-div \cite{Wang19} &
  0.27 &
  0.46 &
  0.81 &
  0.89 &
  0.43 &
  0.75 &
  1.17 &
  1.33 &
  0.54 &
  1.05 &
  1.40 &
  1.56 &
  0.27 &
  0.55 &
  1.16 &
  1.41 &
  0.54 &
  0.78 &
  1.07 &
  1.14 &
  0.29 &
  0.48 &
  0.87 &
  1.04 \\
DCT-RNN-GCN \cite{Mao20DCT} &
  0.25 &
  0.43 &
  0.60 &
  0.69 &
  0.35 &
  0.60 &
  0.95 &
  1.14 &
  0.53 &
  1.01 &
  1.31 &
  1.43 &
  0.19 &
  0.46 &
  1.09 &
  1.35 &
  0.42 &
  0.65 &
  1.00 &
  1.07 &
  0.29 &
  0.47 &
  0.83 &
  1.01 \\ \cline{1-25}
\multicolumn{1}{|c|}{Ours} &
  \textbf{0.22} &
  \textbf{0.30} &
  \textbf{0.47} &
  \textbf{0.50} &
  \textbf{0.27} &
  \textbf{0.44} &
  \textbf{0.67} &
  \textbf{0.76} &
  \textbf{0.34} &
  \textbf{0.67} &
  \textbf{0.96} &
  \textbf{1.07} &
  \textbf{0.18} &
  \textbf{0.34} &
  \textbf{0.65} &
  \textbf{0.77} &
  \textbf{0.38} &
  \textbf{0.54} &
  \textbf{0.72} &
  \textbf{0.79} &
  \textbf{0.22} &
  \textbf{0.33} &
  \textbf{0.53} &
  \textbf{0.62} \\ \bottomrule
\end{tabular}}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|cccc|cccc|cccc|}
\cline{2-25}
\multicolumn{1}{l|}{} &
  \multicolumn{4}{c|}{Sitting Down} &
  \multicolumn{4}{c|}{Taking Photo} &
  \multicolumn{4}{c|}{Waiting} &
  \multicolumn{4}{c|}{Walking Dog} &
  \multicolumn{4}{c|}{Walking Together} &
  \multicolumn{4}{c|}{Average} \\ \hline
\multicolumn{1}{|c|}{\textit{ms}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} &
  {\ul \textit{80}} &
  {\ul \textit{160}} &
  {\ul \textit{320}} &
  {\ul \textit{400}} \\ \cline{1-25}
LTD-10-10 \cite{Mao19LTD} &
  0.30 &
  0.61 &
  0.90 &
  1.00 &
  \textbf{0.14} &
  0.34 &
  0.58 &
  0.70 &
  0.23 &
  0.50 &
  0.91 &
  1.14 &
  0.46 &
  0.79 &
  1.12 &
  1.29 &
  0.15 &
  0.34 &
  0.52 &
  0.57 &
  0.27 &
  0.52 &
  0.83 &
  0.95 \\
BC+WGAIL-div \cite{Wang19} &
  0.34 &
  0.68 &
  1.01 &
  1.14 &
  0.17 &
  0.37 &
  0.60 &
  0.72 &
  0.25 &
  0.53 &
  0.96 &
  1.19 &
  0.46 &
  0.80 &
  1.12 &
  1.31 &
  0.19 &
  0.41 &
  0.61 &
  0.64 &
  0.31 &
  0.57 &
  0.90 &
  1.02 \\
DCT-RNN-GCN \cite{Mao20DCT} &
  0.30 &
  0.63 &
  0.92 &
  1.04 &
  0.16 &
  0.36 &
  0.58 &
  0.70 &
  0.22 &
  0.49 &
  0.92 &
  1.14 &
  0.46 &
  0.78 &
  1.05 &
  1.23 &
  \textbf{0.14} &
  0.32 &
  0.50 &
  0.55 &
  0.27 &
  0.52 &
  0.82 &
  0.94 \\ \cline{1-25}
\multicolumn{1}{|c|}{Ours} &
  \textbf{0.23} &
  \textbf{0.41} &
  \textbf{0.62} &
  \textbf{0.74} &
  \textbf{0.14} &
  \textbf{0.23} &
  \textbf{0.39} &
  \textbf{0.46} &
  \textbf{0.19} &
  \textbf{0.32} &
  \textbf{0.55} &
  \textbf{0.66} &
  \textbf{0.37} &
  \textbf{0.60} &
  \textbf{0.85} &
  \textbf{0.93} &
  0.15 &
  \textbf{0.23} &
  \textbf{0.37} &
  \textbf{0.41} &
  \textbf{0.23} &
  \textbf{0.37} &
  \textbf{0.58} &
  \textbf{0.65} \\ \bottomrule
\end{tabular}}
\caption{Short term, angle on Human3.6}
\label{tab:short_ang}
\end{table*}
